Spatially-Adaptive Reconstruction in Computed Tomography using Neural Networks

We propose a supervised machine learning approach for boosting existing signal and image recovery methods and demonstrate its efficacy on example of image reconstruction in computed tomography. Our technique is based on a local nonlinear fusion of several image estimates, all obtained by applying a chosen reconstruction algorithm with different values of its control parameters. Usually such output images have different bias/variance trade-off. The fusion of the images is performed by feed-forward neural network trained on a set of known examples. Numerical experiments show an improvement in reconstruction quality relatively to existing direct and iterative reconstruction methods.

==> Figures/README <==
$Id: README 17507 2010-03-19 22:52:56Z karl $
This file is public domain.  (Originally written by Karl Berry, 2009.)

This is the README for the epstopdf script distribution.

Primary distribution point: http://mirror.ctan.org/support/epstopdf/
  (list of mirrors at: http://ctan.org/mirrors)

Home page: http://tug.org/epstopdf/

Mailing list for bugs and discussion: http://lists.tug.org/tex-k
When reporting bugs, please include an input file and command line
options, so the problem can be reproduced.

-------------------------------------------------------------------------
The test-binary and test-bin2 files were supplied by Akira Kakuto and
Reinhard Kotucha.  They contain binary data.  They are public domain.

The test-binhdr* files were supplied by Martin von Gagern, constructed
as follows.  They contain binary junk before the EPS starts.  We also
use these to test different line endings.  These files are public domain.

{ echo -e '%Some\000binary\001comment'; dot -Tps <<< 'digraph{a->b}'; }
  > test-binhdr-lf.eps
tr $'\n' $'\r' <test-binhdr-lf.eps >test-binhdr-cr.ps
unix2dos <test-binhdr-lf.eps >test-binhdr-cr.ps


==> Figures/epstopdf.1 <==
.TH EPSTOPDF 1 "28 September 2013"
.\" $Id: epstopdf.1 31784 2013-09-27 22:43:16Z karl $
.SH NAME
epstopdf, repstopdf \- convert an EPS file to PDF
.SH SYNOPSIS
\fBepstopdf\fP [\fIoptions\fP] [\fIepsfile\fP]
.SH DESCRIPTION
\fBepstopdf\fP transforms the Encapsulated PostScript file \fIepsfile\fP
(or standard input) so that it is guaranteed to start at the 0,0
coordinate, and it sets a page size exactly corresponding to the
BoundingBox.  Thus, the result needs no cropping, and the PDF MediaBox
is correct.  By default, the input is converted to PDF using Ghostscript.
.PP
PJL commands at the start of a file are removed.  DOS EPS binary files
(TN 5002) are supported.
.PP
If the bounding box in the input file is not right, of course there will
be resulting problems.
.SH OPTIONS
Options may start with either "\fB-\fP" or "\fB--\fP", and may be
unambiguously abbreviated.  It is best to use the full option name in
scripts, though, to avoid possible collisions with new options in the
future.
.PP
General script options:
.IP "\fB--help\fP
display help message and exit
.IP "\fB--version\fP
display version information and exit
.IP "\fB--outfile\fP=\fIfile\fP"
write result to \fIfile\fP.  If this option is not given, and
\fB--nogs\fP or \fB--filter\fP is specified, write to standard output;
otherwise, the default is to construct the output file name by replacing
any extension in the input file with `.pdf'.
.IP "\fB--\fP[\fBno\fP]\fBdebug\fP"
write debugging info (default: off).
.IP "\fB--\fP[\fBno\fP]\fBexact\fP"
scan ExactBoundingBox (default: off).
.IP "\fB--\fP[\fBno\fP]\fBfilter\fP"
read standard input and (unless \fB--outfile\fP is given) write standard
output (default: off).
.IP "\fB--\fP[\fBno\fP]\fBgs\fP"
run Ghostscript (default: on).  With \fB--nogs\fP, output (to standard
output by default) the PostScript that would normally be converted; that
is, the input PostScript as modified by \fBepstopdf\fP.
.IP "\fB--\fP[\fBno\fP]\fBhires\fP"
scan HiresBoundingBox (default: off).
.IP "\fB--restricted\fP=\fIval\fP"
turn on restricted mode (default: [on for repstopdf, else off]);
this forbids the use of \fB--gscmd\fP and \fB--gsopt\fP and imposes
restrictions on the input and output file names according to the values
of openin_any and openout_any (see the Web2c manual, http://tug.org/web2c).
.PP
Options for Ghostscript (more info below):
.IP "\fB--gscmd\fP=\fIval\fP"
pipe output to \fIval\fP (default: [\fBgswin32c\fP on Windows, else \fBgs\fP])
.IP "\fB--gsopt\fP=\fIval\fP"
include \fIval\fP as one argument in the gs command (can be repeated),
.IP "\fB--gsopts\fP=\fIval\fP"
split \fIval\fP at whitespace, include each resulting word as an
argument in the gs command (can be repeated)
.IP "\fB--autorotate\fP=\fIval\fP"
set AutoRotatePages (default: None); recognized \fIval\fP choices:
None, All, PageByPage.  For EPS files, PageByPage is equivalent to All.
.IP "\fB--\fP[\fBno\fP]\fBcompress\fP"
use compression in the output (default: on).
.IP "\fB--device\fP=\fIdev\fP"
use -sDEVICE=\fIdev\fP (default: pdfwrite); not all devices are allowed
in restricted mode.
.IP "\fB--\fP[\fBno\fP]\fBembed\fP"
embed fonts (default: on).
.IP "\fB--pdfsettings\fP=\fIval\fP"
use -dPDFSETTINGS=/\fIval\fP (default is `prepress' if \fB--embed\fP,
else empty); recognized \fIval\fP choices: screen, ebook, printer,
prepress, default.
.IP "\fB--\fP[\fBno\fP]\fBquiet\fP"
use -q, a.k.a. -dQUIET (default: off).
.IP "\fB--res\fP=\fIdpi, dpi\fPx\fIdpi\fP"
set image resolution (default: [use gs default]); ignored if
\fB--debug\fP is set.
.IP "\fB--\fP[\fBno\fP]\fBsafer\fP"
use -d(NO)QUIET (default: true).
.PP
In addition to the specific options above, additional options to be used
with gs can be specified with either or both of the two cumulative
options \fB--gsopts\fP and \fB--gsopt.\fP
.PP
\fB--gsopts\fP takes a single string of options, which is split at
whitespace, each resulting word then added to the gs command line
individually.
.PP
\fB--gsopt\fP adds its argument as a single option to the gs command
line.  It can be used multiple times to specify options separately,
and is necessary if an option or its value contains whitespace.
.PP
In restricted mode, options are limited to those with names and values
known to be safe; some options taking booleans, integers or fixed
names are allowed, those taking general strings are not.

.SH EXAMPLES
Examples all equivalently producing `test.pdf':
.nf
epstopdf test.eps
cat test.eps | epstopdf --filter >test.pdf
cat test.eps | epstopdf -f -d -o=test.pdf
.fi
.PP
Example to look for HiResBoundingBox and produce corrected PostScript:
.nf
epstopdf -d --nogs --hires test.ps >testcorr.ps 
.fi
.SH BUGS
The case of "%%BoundingBox: (atend)" when input is not seekable (e.g.,
from a pipe) is not supported.
.PP
Report bugs in the program or this man page to tex-k@tug.org.  When
reporting bugs, please include an input file and the command line
options specified, so the problem can be reproduced.
.SH SEE ALSO
\fBgs\fP(1),
\fBpdfcrop\fP(1).
.PP
The epstopdf LaTeX package, part of the oberdiek bundle, which automates
running this script on the fly under TeX: http://ctan.org/pkg/epstopdf-pkg.
.SH AUTHOR
Originally written by Sebastian Rahtz, for Elsevier Science, with
subsequent contributions from Thomas Esser, Gerben Wierda, Heiko
Oberdiek, and many others.  Currently maintained by Karl Berry.
.PP
Man page originally written by Jim Van Zandt.
.PP
epstopdf home page: http://tug.org/epstopdf.
.PP
You may freely use, modify and/or distribute this file.

